MaxStyle: Adversarial Style Composition for Robust Medical Image Segmentation

Convolutional neural networks (CNNs) have achieved remarkable segmentation accuracy on benchmark datasets where training and test sets are from the same domain, yet their performance can degrade significantly on unseen domains, which hinders the deployment of CNNs in many clinical scenarios. Most existing works improve model out-of-domain (OOD) robustness by collecting multi-domain datasets for training, which is expensive and may not always be feasible due to privacy and logistical issues. In this work, we focus on improving model robustness using a single-domain dataset only. We propose a novel data augmentation framework called MaxStyle, which maximizes the effectiveness of style augmentation for model OOD performance. It attaches an auxiliary style-augmented image decoder to a segmentation network for robust feature learning and data augmentation. Importantly, MaxStyle augments data with improved image style diversity and hardness, by expanding the style space with noise and searching for the worst-case style composition of latent features via adversarial training. With extensive experiments on multiple public cardiac and prostate MR datasets, we demonstrate that MaxStyle leads to significantly improved out-of-distribution robustness against unseen corruptions as well as common distribution shifts across multiple, different, unseen sites and unknown image sequences under both low- and high-training data settings. The code can be found at https://github.com/cherise215/MaxStyle.

==> novelty_statement.tex <==
% Statement of Novelty/Impact: This statement, of up to 500 characters in length, should provide the main argument for the inclusion of the paper in the conference. It should clarify whether the main significance of the contribution is in the novelty of the proposed methodology or the scientific/clinical impact of the conclusions or results. Note that this statement will be visible to reviewers and area chairs and should not identify the authors or their institutions.

%% 500 char.
 We present a novel, powerful data augmentation framework (MaxStyle) for single domain generalization, which generates diverse stylized images via adversarial style composition in the feature space for robust learning. It leads to significantly improved model robustness against various unseen distribution shifts at deployment, even when the training data is very limited. As a plug-in module, MaxStyle can be used as an advanced building block for model robustness across various applications.

==> tables/cardiac_high_data.tex <==
\begin{table}[t]
\centering
\caption{Evaluation results on cardiac cross-domain test sets with models trained using 70 ACDC subjects. Reported values are average Dice scores.}
\label{tab:ACDC-high}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}l|c|c|rrr@{}}
\toprule
Method & Intra-domain & OOD & \textit{ACDC-C} & \textit{Cross-site } & \textit{Cross-sequence} \\ \midrule
Baseline & 0.8820 & 0.7197 & 0.7788 & 0.7827 & 0.5974 \\\midrule
RandConv & - & & & & \\
Adv Noise & - & - & - & - & - \\
Adv Bias & - & - & - & - & - \\ \midrule
RSC & 0.8844 & 0.7379 & 0.7757 & 0.8115 & 0.6267 \\
Mixstyle & - & & & & \\
DSU & 0.8784 & 0.7553 & 0.8031 & 0.8126 & 0.6503 \\\midrule
LSM & 0.8740 & 0.7484 & 0.8201 & 0.7954 & 0.6296 \\
\textbf{MaxStyle} & 0.8792 & \textbf{0.8073 }& \textbf{0.8387} & \textbf{0.8330 }& \textbf{0.7501 }\\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/cardiac_low_data_results.tex <==
\begin{table}[t]
\centering
\caption{Evaluation results cardiac cross-domain test sets. OOD: average performance across ACDC-C, cross-site, and cross-sequence datasets. Models are all trained with 10 subjects only. Reported values are average Dice scores over three runs using different seeds and different training sets. }
\label{tab:ACDC-small}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}l|c|c|rrr@{}}
\toprule
Method & Intra-domain & OOD & \textit{ACDC-C} & \textit{Cross-site } & \textit{Cross-sequence} \\ \midrule
Baseline & 0.8108 & 0.5925 \textcolor{gray}{(-)} & 0.6788 & 0.6741 & 0.4244 \\ \midrule
% Mixup & 0.8046 & 0.5581 -3.75% \\
%  & 0.6719 & 0.6691 & 0.3698 \\
RandConv & 0.7729 & 0.6419~\textcolor{gray}{(+8\%)} & 0.6687 & 0.7083 & 0.5486 \\
Adv Noise & 0.7966 & 0.5600~\textcolor{gray}{($-5\%$)}& 0.6778 & 0.6516 & 0.3507 \\
Adv Bias & 0.8114 & 0.6594~\textcolor{gray}{(+11\%)} & 0.6937 & 0.7517 & 0.5327 \\\midrule
% Manifold Mixup & 0.7931 & 0.5787 & 0.6649 & 0.6754 & 0.3958 \\
RSC & 0.8169 & 0.6252~\textcolor{gray}{(+6\%)} & 0.7010 & 0.7015 & 0.4729 \\
MixStyle & 0.8024 & 0.6263~\textcolor{gray}{(+6\%)} & 0.7002 & 0.6984 & 0.4804 \\
DSU & 0.8127 & 0.6088~\textcolor{gray}{(+3\%)} &  0.6972 & 0.7008 & 0.4285  \\ \midrule
LSM & 0.7899 & 0.6462~\textcolor{gray}{(+9\%)} & 0.7221 & 0.7015 & 0.5149 \\
% MaxStyle (the proposed) & 0.8131 & \textbf{0.7453} & \textbf{0.7788} & \textbf{0.7664} & \textbf{0.6909} \\ 
\textbf{MaxStyle} &
\textbf{0.8178} & \textbf{0.7461}~\textcolor{gray}{(+26\%)}  &\textbf{ 0.7789} & \textbf{0.7757} & \textbf{0.6836} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/combined_table.tex <==
\begin{table}[t]
\begin{minipage}{.49\textwidth}
\caption{XXX.}
%Results with highest scores in each category are represented by bold font. }
\label{tab:A}
\begin{adjustbox}{width=0.8\textwidth}
\begin{threeparttable}
\begin{tabular}{@{}lcrr@{}}
\toprule
\multirow{2}{*}{Setting} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{\#  labelled subjects} \\
 & \multicolumn{1}{c}{} & 1 & 3 \\ \midrule
\multirow{5}{*}{Supervised} 
 & {No Aug} & 0.293 & 0.544 \\
& Rand Aug & 0.560 & 0.796 \\ \cmidrule(l){2-4} 
 & +Mixup\cite{Zhang_2018_ICLR_mixup} & 0.575 & 0.801 \\
 & +VAT\cite{Miyato_2018_PAMI_VAT} & 0.570 & 0.811 \\
 & +\textbf{Adv Bias } & \textbf{0.650} & \textbf{0.826} \\ \midrule
\multirow{3}{*}{Semi-supervised} & +VAT\cite{Miyato_2018_PAMI_VAT} & 0.625 & 0.826 \\
 & +\textbf{Adv Bias} & 0.692 & \textbf{0.830} \\ \cmidrule(l){2-4} 
 & cGANs\cite{Chaitanya_2019_IPMI} & \textbf{0.710} & 0.823 \\ \bottomrule
\end{tabular}
\end{threeparttable}
\end{adjustbox}
\end{minipage}
\hfill
\begin{minipage}{.48\textwidth}
\centering
\caption{Segmentation performance of the proposed method and baseline methods across five populations. All were trained with NOR cases only.}
\label{tab:cross_population}
\begin{adjustbox}{width=0.9\textwidth}
\begin{threeparttable}
\begin{tabular}{@{}lccccr@{}}
\toprule
Population & Rand Aug & +Mixup & +VAT & \begin{tabular}[c]{@{}c@{}}+\textbf{Adv Bias} \\ (Proposed)\end{tabular} \\  \midrule
{NOR} & 0.911 & 0.901 & 0.909 & \textbf{0.912} \\ \midrule
{ DCM} & 0.831 & 0.803 & 0.843 & \textbf{0.871} \\
{ HCM} & 0.871 & 0.881 & \textbf{0.891} & 0.890 \\
{ MINF} & 0.805 & 0.789 & 0.824 & \textbf{0.847} \\
{ ARV} & 0.843 & 0.844 & 0.843 &\textbf{ 0.853} \\ \midrule
Average & 0.841 & 0.833 & 0.853 &\textbf{ 0.868} \\ \bottomrule
\end{tabular}


% \begin{tablenotes}
% \item Reported values are average Dice scoresfor the left ventricular myocardium segmentation evaluated on five different populations. Results with highest scores are represented by bold font.
% \end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{minipage}
\end{table}


==> tables/combined_test.tex <==
\begin{table}[htbp]
\begin{minipage}{.7\textwidth}
\renewcommand\arraystretch{0.7}
\caption{Evaluation results cardiac cross-domain test sets. OOD: average performance across ACDC-C, cross-site, and cross-sequence datasets. Models are all trained with 10 subjects only. Reported values are average Dice scores over three runs using different seeds and different training sets. }
\label{tab:ACDC-small}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|c|c|ccc@{}}
\toprule
Method & Intra-domain & OOD & \textit{ACDC-C} & \textit{Cross-site } & \textit{Cross-sequence} \\ \midrule
Baseline & 0.8108 & 0.5925 & 0.6788 & 0.6741 & 0.4244 \\ \midrule
Mixup & 0.8046 & 0.5581 & 0.6719 & 0.6691 & 0.3698 \\
RandConv & 0.7729 & 0.6419 & 0.6687 & 0.7083 & 0.5486 \\
Adv Noise & 0.7966 & 0.5600 & 0.6778 & 0.6516 & 0.3507 \\
Adv Bias & 0.8114 & 0.6594 & 0.6937 & 0.7517 & 0.5327 \\\midrule
Manifold Mixup & 0.7931 & 0.5787 & 0.6649 & 0.6754 & 0.3958 \\
RSC & 0.8169 & 0.6252 & 0.7010 & 0.7015 & 0.4729 \\
MixStyle & 0.8024 & 0.6263 & 0.7002 & 0.6984 & 0.4804 \\
DSU & 0.8127 & 0.6088 & 0.6972 & 0.7008 & 0.4285  \\ \midrule
LSM & 0.7899 & 0.6462 & 0.7221 & 0.7015 & 0.5149 \\
MaxStyle (the proposed) &
\textbf{0.8178} & \textbf{0.7461} &\textbf{ 0.7789} & \textbf{0.7757} & \textbf{0.6836} \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\hfill
\begin{minipage}{.29\textwidth}
    \renewcommand\arraystretch{0.5}
        \begin{tabular}{cccc}
            & \multicolumn{2}{c}{Reali} \\
            & Regolari & Fragili \\
            \midrule
            0& 3247 & 721\\
            1& 253 & 779\\
            \hline
        \end{tabular}

\bigskip

        \begin{tabular}{cccc}
            & \multicolumn{2}{c}{Reali} \\
            & Regolari & Fragili \\
            \midrule
            0& 9931 & 14\\
            1& 47 & 7\\
            \hline
        \end{tabular}
    \end{minipage}
\end{table}


==> todo.tex <==
% 1. change Figure 1 with an explanatory figure. move D to supplementary.
% 2. Equation 5, add under brackets if space allows
% 3. Table 1, simply, put detailed one into supplementary.
% 4. add limitations
5. conduct p-value test
6. provide data links in the reference

